Parametric and Multivariate Uncertainty Calibration for Regression and Object Detection

Reliable spatial uncertainty evaluation of object detection models is of special interest and has been subject of recent work. In this work, we review the existing definitions for uncertainty calibration of probabilistic regression tasks. We inspect the calibration properties of common detection networks and extend state-of-the-art recalibration methods. Our methods use a Gaussian process (GP) recalibration scheme that yields parametric distributions as output (e.g. Gaussian or Cauchy). The usage of GP recalibration allows for a local (conditional) uncertainty calibration by capturing dependencies between neighboring samples. The use of parametric distributions such as as Gaussian allows for a simplified adaption of calibration in subsequent processes, e.g., for Kalman filtering in the scope of object tracking. In addition, we use the GP recalibration scheme to perform covariance estimation which allows for post-hoc introduction of local correlations between the output quantities, e.g., position, width, or height in object detection. To measure the joint calibration of multivariate and possibly correlated data, we introduce the quantile calibration error which is based on the Mahalanobis distance between the predicted distribution and the ground truth to determine whether the ground truth is within a predicted quantile. Our experiments show that common detection models overestimate the spatial uncertainty in comparison to the observed error. We show that the simple Isotonic Regression recalibration method is sufficient to achieve a good uncertainty quantification in terms of calibrated quantiles. In contrast, if normal distributions are required for subsequent processes, our GP-Normal recalibration method yields the best results. Finally, we show that our covariance estimation method is able to achieve best calibration results for joint multivariate calibration.

==> chapter/research.tex <==
\section{Further research}
In the scope of uncertainty calibration, we work with models that output an uncertainty quantification for each forecast. We distinguish between \textit{epistemic} model uncertainty and \textit{aleatoric} data uncertainty \cite{Kendall2017}. Epistemic uncertainty can be assessed using Bayesian methods like Monte-Carlo dropout \cite{Gal2016} or deep ensembles \cite{Lakshminarayanan2017}. In contrast, aleatoric uncertainty is commonly estimated by extending a forecaster to directly output a parameterized distribution (e.g. Gaussian) \cite{Kendall2017,He2019,Hall2020,Harakeh2020,Feng2021}. A different branch of yielding prediction uncertainties is quantile regression where a forecaster outputs estimates for certain quantile levels \cite{Fasiolo2020,Chung2021}. The advantage of quantile regression is that no parametric assumptions about the output distribution is necessary. However, these methods haven't been used for object detection so far, thus, we focus on detection models that output a parametric estimate for the object position \cite{He2019,Hall2020,Harakeh2020,Feng2021}.

Besides their definition of \textit{quantile calibration}, the authors in \cite{Kuleshov2018} propose to use the isotonic regression calibration method \cite{Zadrozny2002} from classification calibration to recalibrate the cumulative distribution function predicted by a probabilistic forecaster. Similar to this approach, the authors in \cite{Song2019} use beta calibration \cite{Kull2017} in conjunction with Gaussian process (GP) parameter estimation to recalibrate the cumulative distribution and to achieve \textit{distribution calibration}. Both approaches exploit the fact that the cumulative is defined in the $[0, 1]$ interval which allows for an application of recalibration methods from the scope of classification calibration. While the former method \cite{Kuleshov2018} seeks for the optimal recalibration parameters globally, the latter approach \cite{Song2019} utilizes GP parameter estimation to find the optimal recalibration parameters for a single distribution using all samples whose distribution moments are close to the target sample.
%\textcolor{red}{Versteh ich nicht. Also wirklich alle Samples mit Momenten matchen und dann mit EINEM target sample vergleichen?} 
This allows for a local uncertainty recalibration. In contrast, the authors in \cite{Levi2019} and \cite{Laves2020} perform \textit{variance calibration} and use temperature scaling \cite{Guo2018} to rescale the variance of a normal distribution. This method optimizes the negative log likelihood (NLL) to find the optimal rescaling parameter. As opposed to post-hoc calibration, there are also methods that aim to achieve regression calibration during model training, e.g., calibration loss \cite{Feng2019}, maximum mean discrepancy (MMD) \cite{Cui2020} or $f$-Cal \cite{Bhatt2021}. The former approach adds a loss term to match the predicted variances with the observed squared error, while the latter methods introduce a second loss term to perform distribution matching during model training. The advantage of these approaches is that an additional calibration data set is not needed. However, it is necessary to retrain the whole network architecture. Thus, we focus on post-hoc calibration methods in this work. 
